GRAC: Self-Guided and Self-Regularized Actor-Critic

Deep reinforcement learning (DRL) algorithms have successfully been demonstrated on a range of challenging decision making and control tasks. One dominant component of recent deep reinforcement learning algorithms is the target network which mitigates the divergence when learning the Q function. However, target networks can slow down the learning process due to delayed function updates. Our main contribution in this work is a self-regularized TD-learning method to address divergence without requiring a target network. Additionally, we propose a self-guided policy improvement method by combining policy-gradient with zero-order optimization to search for actions associated with higher Q-values in a broad neighborhood. This makes learning more robust to local noise in the Q function approximation and guides the updates of our actor network. Taken together, these components define GRAC, a novel self-guided and self-regularized actor critic algorithm. We evaluate GRAC on the suite of OpenAI gym tasks, achieving or outperforming state of the art in every environment tested.

==> tex/impact.tex <==
This work propose new methods to improve reinforcement learning in continuous control tasks. 
(1) DRL takes a lot of data, thus compute, to train. Our method speeds up training, thus reduces the necessary compute and the corresponding carbon footprint and energy consumption.
(2) DRL's successful application in robotics would have societal impacts. On the positive side, automating repetitive manual labour increases productivity and thus increases the wealth of the society. On the other hand, automation may lead to unemployment of workers who have previously performed this manual labour. New policies are required to ensure decent income and access to professional education, so the impacted workers can transition into newly created jobs.
